Contextuality-by-default for behaviours in compatibility scenarios

We show that the main idea behind contextuality-by-default (CbD), i.e., the assumption that a physical measurement has to be understood as a contextual collection of random variables, is implicit in the compatibility-hypergraph approach to contextuality (CA) and use this result to develop in the latter important concepts which were introduced in the former. We introduce in CA the non-degeneracy condition, which is the analogous of consistent connectedness, and prove that this condition is, in general, weaker than non-disturbance condition. The set of non-degenerate behaviours defines a polytope, implying that one can characterize consistent connectedness using linear inequalities. We introduce the idea of extended contextuality for behaviours and prove that a behaviour is non-contextual in the standard sense iff it is non-degenerate and non-contextual in the extended sense. Finally, we use extended scenarios and behaviours to shed new light on our results.

==> Bibliography.tex <==
% Bibliography in chronological order

@article{bell1964einstein,
  title={On the einstein podolsky rosen paradox},
  author={Bell, John S},
  journal={Physics Physique Fizika},
  volume={1},
  number={3},
  pages={195},
  year={1964},
  publisher={APS}
}

@article{bell1966problem,
  title={On the problem of hidden variables in quantum mechanics},
  author={Bell, John S},
  journal={Reviews of Modern Physics},
  volume={38},
  number={3},
  pages={447},
  year={1966},
  publisher={APS}
}

@incollection{kochen1975problem,
  title={The problem of hidden variables in quantum mechanics},
  author={Kochen, Simon and Specker, Ernst P},
  booktitle={The logico-algebraic approach to quantum mechanics},
  pages={293--328},
  year={1975},
  publisher={Springer}
}

@article{abramsky2011sheaf,
  title={The sheaf-theoretic structure of non-locality and contextuality},
  author={Abramsky, Samson and Brandenburger, Adam},
  journal={New Journal of Physics},
  volume={13},
  number={11},
  pages={113036},
  year={2011},
  publisher={IOP Publishing}
}

@book{brondsted2012introduction,
  title={An introduction to convex polytopes},
  author={Brondsted, Arne},
  volume={90},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@article{araujo2013allnoncontextualityineq,
   title={All noncontextuality inequalities for then-cycle scenario},
   volume={88},
   ISSN={1094-1622},
   url={http://dx.doi.org/10.1103/PhysRevA.88.022118},
   DOI={10.1103/physreva.88.022118},
   number={2},
   journal={Physical Review A},
   publisher={American Physical Society (APS)},
   author={Araújo, Mateus and Quintino, Marco Túlio and Budroni, Costantino and Cunha, Marcelo Terra and Cabello, Adán},
   year={2013},
   month={Aug}
}


@article{dzhafarov2013allpossiblecouplings,
   title={All-Possible-Couplings Approach to Measuring Probabilistic Context},
   volume={8},
   ISSN={1932-6203},
   url={http://dx.doi.org/10.1371/journal.pone.0061712},
   DOI={10.1371/journal.pone.0061712},
   number={5},
   journal={PLoS ONE},
   publisher={Public Library of Science (PLoS)},
   author={Dzhafarov, Ehtibar N. and Kujala, Janne V.},
   editor={Adesso, GerardoEditor},
   year={2013},
   month={May},
   pages={e61712}
}

@misc{dzhafarov2013qualified,
    title={A Qualified Kolmogorovian Account of Probabilistic Contextuality},
    author={Ehtibar N. Dzhafarov and Janne V. Kujala},
    year={2013},
    eprint={1304.4546},
    archivePrefix={arXiv},
    primaryClass={math-ph}
}

@article{dzhafarov2014noforcingnomatching,
   title={No-Forcing and No-Matching Theorems for Classical Probability Applied to Quantum Mechanics},
   volume={44},
   ISSN={1572-9516},
   url={http://dx.doi.org/10.1007/s10701-014-9783-3},
   DOI={10.1007/s10701-014-9783-3},
   number={3},
   journal={Foundations of Physics},
   publisher={Springer Science and Business Media LLC},
   author={Dzhafarov, Ehtibar N. and Kujala, Janne V.},
   year={2014},
   month={Mar},
   pages={248–265}
}



@article{dzhafarov2014embedding,
   title={Embedding Quantum into Classical: Contextualization vs Conditionalization},
   volume={9},
   ISSN={1932-6203},
   url={http://dx.doi.org/10.1371/journal.pone.0092818},
   DOI={10.1371/journal.pone.0092818},
   number={3},
   journal={PLoS ONE},
   publisher={Public Library of Science (PLoS)},
   author={Dzhafarov, Ehtibar N. and Kujala, Janne V.},
   editor={Adesso, GerardoEditor},
   year={2014},
   month={Mar},
   pages={e92818}
}


@article{CSW2014,
  title = {Graph-Theoretic Approach to Quantum Correlations},
  author = {Cabello, Ad\'an and Severini, Simone and Winter, Andreas},
  journal = {Phys. Rev. Lett.},
  volume = {112},
  issue = {4},
  pages = {040401},
  numpages = {5},
  year = {2014},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.112.040401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.112.040401}
}

@phdthesis{amaral2014exclusivity,
  title={The Exclusivity principle and the set o quantum distributions},
  author={Amaral, B},
  year={2014},
  school={ Universidade Federal de Minas Gerais}
}
@article{acin2015combinatorial,
  title={A combinatorial approach to nonlocality and contextuality},
  author={Ac{\'\i}n, Antonio and Fritz, Tobias and Leverrier, Anthony and Sainz, Ana Bel{\'e}n},
  journal={Communications in Mathematical Physics},
  volume={334},
  number={2},
  pages={533--628},
  year={2015},
  publisher={Springer}
}

@article{dzhafarov2015threetypes,
   title={Contextuality in Three Types of Quantum-Mechanical Systems},
   volume={45},
   ISSN={1572-9516},
   url={http://dx.doi.org/10.1007/s10701-015-9882-9},
   DOI={10.1007/s10701-015-9882-9},
   number={7},
   journal={Foundations of Physics},
   publisher={Springer Science and Business Media LLC},
   author={Dzhafarov, Ehtibar N. and Kujala, Janne V. and Larsson, Jan-Åke},
   year={2015},
   month={Mar},
   pages={762–782}
}


@misc{dzhafarov2015contextcontent,
    title={Context-Content Systems of Random Variables: The Contextuality-by-Default Theory},
    author={Ehtibar N. Dzhafarov and Janne V. Kujala},
    year={2015},
    eprint={1511.03516},
    archivePrefix={arXiv},
    primaryClass={math.PR}
}

@article{roch2015modern,
  title={Modern discrete probability: An essential toolkit},
  author={Roch, Sebastien},
  journal={Lecture notes},
  year={2015},
  url = {http://www.math.wisc.edu/~roch/mdp/},
  pages={Chapter 4}
}

@article{kujala2015necessary,
  title = {Necessary and Sufficient Conditions for an Extended Noncontextuality in a Broad Class of Quantum Mechanical Systems},
  author = {Kujala, Janne V. and Dzhafarov, Ehtibar N. and Larsson, Jan-\AA{}ke},
  journal = {Phys. Rev. Lett.},
  volume = {115},
  issue = {15},
  pages = {150401},
  numpages = {5},
  year = {2015},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.115.150401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.115.150401}
}

@article{dzhafarov2016contextsocialsystems,
   title={Is there contextuality in behavioural and social systems?},
   volume={374},
   ISSN={1471-2962},
   url={http://dx.doi.org/10.1098/rsta.2015.0099},
   DOI={10.1098/rsta.2015.0099},
   number={2058},
   journal={Philosophical Transactions of the Royal Society A: Mathematical, Physical and Engineering Sciences},
   publisher={The Royal Society},
   author={Dzhafarov, E. N. and Zhang, Ru and Kujala, Janne},
   year={2016},
   month={Jan},
   pages={20150099}
}


@misc{dzhafarov2016contextualitybydefault,
    title={Contextuality-by-Default 2.0: Systems with Binary Random Variables},
    author={Ehtibar N. Dzhafarov and Janne V. Kujala},
    year={2016},
    eprint={1604.04799},
    archivePrefix={arXiv},
    primaryClass={quant-ph}
}

@misc{cervantes2017snow,
    title={Snow Queen is Evil and Beautiful: Experimental Evidence for Probabilistic Contextuality in Human Choices},
    author={Victor H. Cervantes and Ehtibar N. Dzhafarov},
    year={2017},
    eprint={1711.00418},
    archivePrefix={arXiv},
    primaryClass={q-bio.NC}
}

@article{dzhafarov2017contextualitycanonicalsystems,
   title={Contextuality in canonical systems of random variables},
   volume={375},
   ISSN={1471-2962},
   url={http://dx.doi.org/10.1098/rsta.2016.0389},
   DOI={10.1098/rsta.2016.0389},
   number={2106},
   journal={Philosophical Transactions of the Royal Society A: Mathematical, Physical and Engineering Sciences},
   publisher={The Royal Society},
   author={Dzhafarov, Ehtibar N. and Cervantes, Víctor H. and Kujala, Janne V.},
   year={2017},
   month={Oct},
   pages={20160389}
}


@book{amaral2018graph,
  title={On graph approaches to contextuality and their role in quantum theory},
  author={Amaral, Barbara and Cunha, Marcelo Terra},
  year={2018},
  publisher={Springer},
  doi = {10.1007/978-3-319-93827-1}
}

@article{amaral2018necessaryextended,
   title={Necessary conditions for extended noncontextuality in general sets of random variables},
   volume={59},
   ISSN={1089-7658},
   url={http://dx.doi.org/10.1063/1.5024885},
   DOI={10.1063/1.5024885},
   number={7},
   journal={Journal of Mathematical Physics},
   publisher={AIP Publishing},
   author={Amaral, Barbara and Duarte, Cristhiano and Oliveira, Roberto I.},
   year={2018},
   month={Jul},
   pages={072202}
}

@article{dzhafarov2018somethingspecial,
   title={Replacing Nothing with Something Special: Contextuality-by-Default and Dummy Measurements},
   ISBN={9783319749716},
   ISSN={2520-1948},
   url={http://dx.doi.org/10.1007/978-3-319-74971-6_5},
   DOI={10.1007/978-3-319-74971-6_5},
   journal={Quantum Foundations, Probability and Information},
   publisher={Springer International Publishing},
   author={Dzhafarov, Ehtibar N.},
   year={2018},
   pages={39–44}
}


@article{kujala2019measuresofcontextuality,
   title={Measures of contextuality and non-contextuality},
   volume={377},
   ISSN={1471-2962},
   url={http://dx.doi.org/10.1098/rsta.2019.0149},
   DOI={10.1098/rsta.2019.0149},
   number={2157},
   journal={Philosophical Transactions of the Royal Society A: Mathematical, Physical and Engineering Sciences},
   publisher={The Royal Society},
   author={Kujala, Janne V. and Dzhafarov, Ehtibar N.},
   year={2019},
   month={Sep},
   pages={20190149}
}


@article{amaral2019extendedcontextuality,
   title={Characterizing and quantifying extended contextuality},
   volume={100},
   ISSN={2469-9934},
   url={http://dx.doi.org/10.1103/PhysRevA.100.062103},
   DOI={10.1103/physreva.100.062103},
   number={6},
   journal={Physical Review A},
   publisher={American Physical Society (APS)},
   author={Amaral, Barbara and Duarte, Cristhiano},
   year={2019},
   month={Dec}
}

@article{ACC14,
  title = {Exclusivity principle forbids sets of correlations larger than the quantum set},
  author = {Amaral, Barbara and Cunha, Marcelo Terra and Cabello, Ad\'an},
  journal = {Phys. Rev. A},
  volume = {89},
  issue = {3},
  pages = {030101},
  numpages = {4},
  year = {2014},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.89.030101},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.89.030101}
}

@article{NoncontextualWirings,
  title = {Noncontextual Wirings},
  author = {Amaral, Barbara and Cabello, Ad\'an and Cunha, Marcelo Terra and Aolita, Leandro},
  journal = {Phys. Rev. Lett.},
  volume = {120},
  issue = {13},
  pages = {130403},
  numpages = {6},
  year = {2018},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.120.130403},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.120.130403}
}

